DataTV: Streaming Data Videos for Storytelling

Data videos -- motion graphics that incorporate visualizations -- have been recognized as an effective way to communicate ideas, but creating such video requires both time and expertise, precluding them from being created and streamed live. We introduce DataTV, a system for combining multiple media sources in real time. We validate our work through an expert review involving researchers using the DataTV prototype to create a one-minute data video for their current project. Results show that the new method facilitates rapid creation and enables users to focus on the narrative rather than mechanics of video production.

==> 1-intro.tex <==
% 1-intro.tex
\firstsection{Introduction}

Applying the age-old practice of storytelling to data visualization~\cite{Gershon2001} is one of the most transformative developments in recent history for visualization research~\cite{Kosara2013b}.
As this approach matures, practitioners and researchers alike are adding to the types of storytelling media being used for this purpose~\cite{Segel2010}; beyond the traditional slideshow~\cite{Kosara2013}, recent efforts are now exploring the use of infographics~\cite{Segel2010}, hand-drawn comics~\cite{Bach2016}, and interactive sketching~\cite{Lee2013}.
The use of motion graphics, or so-called \textit{data videos}~\cite{Amini2015}, is particularly interesting as it allows for creating compelling visual narratives using rich multimedia sources, such as live video, graphics, text, sound, and music.
However, authoring effective videos that utilize the medium to its fullest is time-consuming, resource-intensive, and requires a significant amount of skill.
In particular, this precludes such videos from being created and streamed live on the internet.

In this paper, we study how to enable dynamically streaming visual exploration for storytelling.
Such a live ``data TV'' approach will require a streamlined and fully integrated software platform where a single person can prepare, record, and produce the digital stream with a minimum of time investment.
To enable the creation of such live data videos, we propose the \textsc{DataTV} platform, a prototype system for authoring live-streaming data videos using an integrated interface.
The prototype supports three separate modes for (1) production, (2) recording, and (3) editing, in a highly streamlined and optimized workflow that allows a single content creator to control the entire process during live streaming.

To validate the DataTV platform, we asked two visualization experts to create a data video less than one minute long using DataTV on a specific topic to collect real experiences on using the system for storytelling.
Results from this expert review (participant-generated clips are included in the companion video for this paper) indicate that these researchers were impressed with the relative ease they could create these videos.
Interestingly, our findings suggest that the integrated functionality in the DataTV platform enabled the researchers to focus on storytelling rather than the mechanics of video production.
Their overall feedback guided further improvements to the platform.

% \section{Data Information to Data Videos}
% There are examples that data stories, shown as data visualization blended in videos and documentaries. The examples revealed that the data visualization were capable of delivering important information.

% The contributions of our work are the following:
% \begin{enumerate}
% \item The notion of \textit{live data videos} for streaming real-time data analysis to an internet audience;
% \item A prototype \textit{integrated platform} for real-time creation of data videos by combining multiple sources of information including visualizations, websites, and multimedia; and
% \item Results from an \textit{expert review} suggesting that our prototype facilitates creating data videos by relieving storytellers from the mechanics of video production.
% \end{enumerate}

